Completeness of the NASA/IPAC Extragalactic Database (NED) -- Local Volume Sample

We introduce the NASA/IPAC Extragalactic Database (NED) Local Volume Sample (NED-LVS), a subset of $\sim$1.9 million objects with distances out to 1000~Mpc. We use UV and IR fluxes available in NED from all-sky surveys to derive physical properties, and estimate the completeness relative to the expected local luminosity density. The completeness relative to NIR luminosities (which traces a galaxy's stellar mass) is roughly 100% at $D<$30~Mpc and remains moderate (70%) out to 300~Mpc. For brighter galaxies ($\gtrsim L^{*}$), NED-LVS is $\sim$100% complete out to $\sim$400~Mpc. When compared to other local Universe samples (GLADE and HECATE), all three are $\sim$100% complete below 30~Mpc. At distances beyond $\sim$80~Mpc, NED-LVS is more complete than both GLADE and HECATE by $\sim$10-20%. NED-LVS is the underlying sample for the NED gravitational wave follow-up (NED-GWF) service, which provides prioritized lists of host candidates for GW events within minutes of alerts issued by the LIGO-Virgo-KAGRA collaboration. We test the prioritization of galaxies in the volume of GW170817 by 3 physical properties, where we find that both stellar mass and inverse specific star formation rate place the correct host galaxy in the top ten. In addition, NED-LVS can be used for a wide variety of other astrophysical studies: galaxy evolution, star formation, large-scale structure, galaxy environments, and more. The data in NED are updated regularly, and NED-LVS will be updated concurrently. Consequently, NED-LVS will continue to provide an increasingly complete sample of galaxies for a multitude of astrophysical research areas for years to come.

==> tables/2mpzVischk.tex <==
\begin{table*}


{Closely Grouped Stars Misclassified as Galaxies}\\
\begin{tabular}{lrrrcc}

\hline
\hline
Object         & RA      &  Dec      & |b|    & Obj Type   & Obj Type    \\ 
Name           & (De)    &  (FUV)    & (Deg)  & (old)     & (new)                  \\ 
               & (J2000) &  (J2000)  &        &                 &                  \\ 
\hline

WISEA J080224.37$-$303407.0 & 120.6016 & -30.5686 & 0.09 & G & Star \\
WISEA J071342.81$-$173834.9 & 108.4284 & -17.6430 & -3.20 & G & Star \\
WISEA J064018.78$-$015124.9 & 100.0782 & -1.8571 & -3.32 & G & Star \\
WISEA J060539.96+051012.7 & 91.4165 & 5.1702 & -7.74 & G & Star \\
WISEA J053732.60+241454.9 & 84.3854 & 24.2485 & -4.01 & G & Star \\
WISEA J211614.80+382620.3 & 319.0618 & 38.4389 & -7.37 & G & Star \\
WISEA J050752.76+323535.5 & 76.9700 & 32.5933 & -4.69 & G & Star \\
WISEA J191108.41+245723.0 & 287.7851 & 24.9561 & 7.07 & G & Star \\
WISEA J221412.11+492211.6 & 333.5505 & 49.3698 & -5.87 & G & Star \\
WISEA J044800.71+464619.9 & 72.0031 & 46.7722 & 1.12 & G & Star \\
\hline

\end{tabular}

\input{tables/2mpzVischk.txt}
\label{tab:2mpzVischk}


\end{table*}


==> tables/ColDesc_back.tex <==
\begin{table*}

{Description of NED-LVS Columns} \\
\begin{tabular}{l@{\hskip -1.1cm}r@{\hskip 0.1cm}rp{11cm}}

\hline
\hline
 Column  & Data Type & Unit & Description      \\

\hline

objname & S & -- & Prefered object name in NED \\
ra & D & deg & Right ascension [J2000] \\
dec & D & deg & Declination [J2000] \\
objtype & S & -- & Prefered object type in NED (see Table 1 in section 2.1) \\
objtype\_flag & B & -- & Boolean flag indicating that the objtype has been updated in NED-LVS \\
z, z\_unc & F & -- & Fiducial redshift [heliocentric] \\
z\_tech & S & -- & Technique used to measure redshift [SPEC, PHOT, UNKN, INFD, MOD, NULL] \\
z\_qual & B & -- & Qualifier flag indicating reliability of redshift [True=unreliable] \\
z\_qual\_flag & B & -- & Boolean flag indicating that the zqual flag has been updated in NED-LVS \\
z\_refcode & S & -- & Reference code for the publication that provided the redshift \\
ziDist, ziDist\_unc & F & Mpc & Redshift-independent distance computed as the weighted average of measurements in either the primary or secondary indicators \\
ziDist\_method & S & -- & Method used to measure the redshift-independent distance when a single method is used to compute the weighted average, otherwise "Wavg" when a mixture of methods are used [Cepheid, SNIa, TRGB, Wavg, etc.] \\
ziDist\_Indicator & S & -- & Measurement type indicator for redshift-independent distance [Primary or Secondary] \\
ziDist\_refcode & S & -- & Reference code for the publication that provided the distance when a single measurement was chosen, otherwise "Mix" indicates an average of multiple measurements was used [refcode or Mix] \\
DistMpc, DistMpc\_unc & F & Mpc & Selected distance used in NED-LVS \\
DistMpc\_method & S & -- & Method used in the selected distance [Redshift or zIndependent] \\
ebv & F & mag & Foreground MW reddening E(B-V) from Schlafly \& Finkbeiner (2011) \\
A\_FUV\_MWext & F & mag & MW extinction in GALEX FUV-band assuming Fitzpatrick et al. (1999) \\
A\_NUV\_MWext & F & mag & MW extinction in GALEX NUV-band assuming Fitzpatrick et al. (1999) \\
A\_J\_MWext & F & mag & MW extinction in 2MASS J-band assuming Fitzpatrick et al. (1999) \\
A\_H\_MWext & F & mag & MW extinction in 2MASS H-band assuming Fitzpatrick et al. (1999) \\
A\_Ks\_MWext & F & mag & MW extinction in 2MASS Ks-band assuming Fitzpatrick et al. (1999) \\
A\_W1\_MWext & F & mag & MW extinction in WISE W1-band assuming Fitzpatrick et al. (1999) \\
A\_W2\_MWext & F & mag & MW extinction in WISE W2-band assuming Fitzpatrick et al. (1999) \\
A\_W3\_MWext & F & mag & MW extinction in WISE W3-band assuming Fitzpatrick et al. (1999) \\
A\_W4\_MWext & F & mag & MW extinction in WISE W4-band assuming Fitzpatrick et al. (1999) \\
m\_J, m\_J\_unc & F & mag & Apparent magnitude in 2MASS J-band  in Vega system \\
m\_H, m\_H\_unc & F & mag & Apparent magnitude in 2MASS H-band  in Vega system \\
m\_Ks, m\_Ks\_unc & F & mag & Apparent magnitude in 2MASS Ks-band  in Vega system \\
tMASSphot & S & -- & Flag indicating which catalog was used for 2MASS photometry [PSC, XSC, LGA] \\
m\_FUV, m\_FUV\_unc & F & mag & Apparent magnitude in GALEX FUV-band  in AB system \\
m\_NUV, m\_NUV\_unc & F & mag & Apparent magnitude in GALEX NUV-band  in AB system \\
GALEXphot & S & -- & Flag indicating which catalog was used for GALEX photometry [ASC, MSC, z0MGS] \\
m\_W1, m\_W1\_unc & F & mag & Apparent magnitude in WISE W1-band  in Vega system \\
m\_W2, m\_W2\_unc & F & mag & Apparent magnitude in WISE W2-band  in Vega system \\
m\_W3, m\_W3\_unc & F & mag & Apparent magnitude in WISE W3-band  in Vega system \\
m\_W4, m\_W4\_unc & F & mag & Apparent magnitude in WISE W4-band  in Vega system \\
WISEphot & S & -- & Flag indicating which catalog was used for WISE photometry [Pfit, APER, z0MGS] \\
Lum\_FUV, Lum\_FUV\_unc & D & erg/s & Monochromatic luminosity ($\nu*F_{\nu}$) in GALEX FUV-band \\
Lum\_NUV, Lum\_NUV\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in GALEX NUV-band \\
Lum\_J, Lum\_J\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in 2MASS J-band \\
Lum\_H, Lum\_H\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in 2MASS H-band \\
Lum\_Ks, Lum\_Ks\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in 2MASS Ks-band \\
Lum\_W1, Lum\_W1\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in WISE W1-band \\
Lum\_W2, Lum\_W2\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in WISE W2-band \\
Lum\_W3, Lum\_W3\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in WISE W3-band \\
Lum\_W4, Lum\_W4\_unc & D & erg/s & Monochromatic luminosity (nu*F\_nu) in WISE W4-band \\
SFR\_W4, SFR\_W4\_unc & F & Msun/yr & Star formation rate using W4 luminosity scaling relationship (Section 2.4) \\
SFR\_hybrid, SFR\_hybrid\_unc & F & Msun/yr & Star formation rate using a FUV+W4 luminosity scaling relationship (Section 2.4) \\
Mstar, Mstar\_unc & F & Msun & Stellar mass using a W1 luminosity scaling relationship (Section 2.4) \\
MLratio & F & Msun/erg/s & The mass-to-light ratio used to calculate Mstar (Section 2.4) \\
SFR\_flag & B & -- & Boolean flag on SFR measurements to indicate an overestimated value due to early-type galaxy determination based on IR or UV-IR colors (Section 4.3) [True=colors indicate an early-type galaxy] \\
\hline
\end{tabular}

\input{tables/ColDesc.txt}
\label{tab:ColDesc}

\end{table*}


==> tables/gw170817.tex <==
\begin{table*}
\begin{tabular}{lcllcl}


{Galaxy Lists in GW170817 Sky Localizations} \\ 

\hline
\multicolumn{3}{l}{Sky Map w/o Virgo (187~deg$^2$; N_{inVol}=46)} & \multicolumn{3}{l}{Final Sky Map (31~deg$^2$; N_{inVol}=207)} \\ 
\hline


Galaxy & Rank & Log(Mstar) & Galaxy & Rank & Log(Mstar) \\
\hline
NGC 5061 & 1 & 11.12 & NGC 4830 & 1 & 10.78 \\
NGC 4830 & 2 & 10.78 & NGC 4970 & 2 & 10.76 \\
NGC 4970 & 3 & 10.76 & NGC 4763 & 3 & 10.74 \\
NGC 4763 & 4 & 10.74 & IC 4197 & 4 & 10.68 \\
NGC 5114 & 5 & 10.68 & NGC 4993 & 5 & 10.65 \\
IC 4197 & 6 & 10.68 & IC 4180 & 6 & 10.55 \\
NGC 5967 & 7 & 10.65 & NGC 4968 & 7 & 10.41 \\
NGC 4993 & 8 & 10.65 & MCG -02-33-036 & 8 & 10.27 \\
NGC 3976 & 9 & 10.60 & UGCA 331 & 9 & 10.22 \\
NGC 4348 & 10 & 10.57 & ESO 575- G 029 & 10 & 10.06 \\
\\
Galaxy & Rank & Log(SFR) & Galaxy & Rank & Log(SFR) \\
\hline
WISEA J120824.18+030047.7 & 1 & -3.02 & WISEA J125701.31-172324.4 & 1 & -2.46 \\
UGCA 286 & 2 & -2.87 & ESO 575- G 061 & 2 & -2.29 \\
UGCA 289 & 3 & -2.85 & ESO 508- G 035 & 3 & -2.09 \\
LSBC D571-08 & 4 & -2.85 & WISEA J130734.15-234855.6 & 4 & -1.94 \\
MCG -02-32-026 & 5 & -2.81 & WISEA J131426.55-271242.8 & 5 & -1.94 \\
WISEA J112806.20+175913.7 & 6 & -2.79 & WISEA J130730.83-231014.4 & 6 & -1.88 \\
WISEA J123259.84-074956.4 & 7 & -2.77 & UGCA 325 & 7 & -1.85 \\
WISEA J121754.81+002605.5 & 8 & -2.74 & WISEA J131246.73-255912.9 & 8 & -1.85 \\
WISEA J113708.74+131505.2 & 9 & -2.69 & 2MFGC 10461 & 9 & -1.85 \\
WISEA J111052.13+211215.5 & 10 & -2.63 & WISEA J130415.23-225251.0 & 10 & -1.83 \\
\ldots & \ldots &\ldots &\ldots &\ldots &\ldots \\
NGC 4993 & 84 & -1.30 & NGC 4993 & 22 & -1.30 \\
\\
Galaxy & Rank & Log(sSFR) & Galaxy & Rank & Log(sSFR) \\
\hline
NGC 4970 & 1 & -12.57 & NGC 4970 & 1 & -12.57 \\
NGC 4830 & 2 & -12.52 & NGC 4830 & 2 & -12.52 \\
IC 0874 & 3 & -12.25 & NGC 4993 & 3 & -11.94 \\
UGCA 289 & 4 & -12.00 & IC 4197 & 4 & -11.67 \\
NGC 5048 & 5 & -11.98 & ESO 575- G 061 & 5 & -11.31 \\
NGC 4993 & 6 & -11.94 & WISEA J125732.70-194200.8 & 6 & -11.29 \\
NGC 5114 & 7 & -11.92 & 2MFGC 10461 & 7 & -11.29 \\
MCG -02-32-026 & 8 & -11.89 & WISEA J125251.08-152929.7 & 8 & -11.18 \\
NGC 5061 & 9 & -11.83 & IC 4180 & 9 & -11.14 \\
IC 4197 & 10 & -11.67 & UGCA 325 & 10 & -11.02 \\
\hline
\end{tabular}

\input{tables/gw170817.txt}
\label{tab:gw170817}


\end{table*}


==> tables/zcats.tex <==
\begin{table*}
\centering
\begin{tabular}{lrll}
\hline
\hline
Survey Catalog    & \#Redshifts & z Notes & Area\\
\hline
PS1-STRM (Beck et al. 2016) & $2.9\times 10^9$ & $0 < z < 0.5$ & 3 pi \\
DESI (Zou et al. 2019)      & $1.7\times 10^8$ & $0 < z < 1  $ & 3 pi \\
SDSS DR12 (Beck et al. 2016)& $2.1\times 10^8$ &		       & $\rm 9,500~deg^2$ \\
SDSS IV, DR17, eBOSS	    & $5.0\times 10^8$ & Spec-z	       & $\rm 14,555~deg^2$ \\
WISE $\times$ SuperCOSMOS (Bilicki et al. 2016) & $2.0\times 10^7$ & $0 < z < 0.5$	  & 3 pi \\
Subaru HPC-SSP, Deep (Tanaka et al. 2018)& $2.0\times 10^8$ & $0.2 < z < 1.5$ & $\rm 27~deg^2$ \\
LSST	    & $3.7\times 10^9$ & $0.3 < z < 3.0$	       & $\rm 20,005~deg^2$ \\
Euclid DR1	    & $2.5\times 10^8$ & Photo+Spec z's	       & $\rm 2,500~deg^2$ \\
SPHEREx	    & $4.9\times 10^8$ & $0 < z < 3$	       & 4 pi \\

\hline
\end{tabular}
\input{tables/zcats.txt}
\label{tab:zcats}

\end{table*}

==> texstuff/completeness_authors.tex <==
\author
{D.O. Cook$^{1}$,
J.M. Mazzarella$^{1}$,
G. Helou$^{1}$,
A. Alcala$^{1}$,
T.X. Chen$^{1}$,
R. Ebert$^{1}$,
\newauthor
C. Frayer$^{1}$,
J. Kim$^{1}$,
T. Lo$^{1}$,
B.F. Madore$^{2,3}$,
P.M. Ogle$^{4}$,
M. Schmitz$^{1}$,
\newauthor
L.P. Singer$^{5}$,
S. Terek$^{1}$,
J. Valladon$^{6,7}$,
X. Wu$^{1}$,
\\ 
$^{1}$Caltech/IPAC, 1200 E. California Boulevard, Pasadena, CA 91125, USA\\ 
$^{2}$Department of Astronomy \& Astrophysics, University of Chicago, 5640 South Ellis Avenue, Chicago, IL 60637, USA\\ 
$^{3}$Observatories of the Carnegie Institution for Science, Pasadena, CA\\ 
$^{4}$Space Telescope Science Institute, Baltimore, MD\\ 
$^{5}$NASA Goddard Space Flight Center, Code 661, Greenbelt, MD 20771, USA\\ 
$^{6}$Department of Astronomy, San Diego State University, 5500 Campanile Drive, San Diego, CA, 92812-1221, USA\\ 
$^{7}$Dept. of Physics \& Astronomy, San Jose State University, San Jose, CA\\ 
}
